SelMatch: Effectively Scaling Up Dataset Distillation via Selection-Based Initialization and Partial Updates by Trajectory Matching

Dataset distillation aims to synthesize a small number of images per class (IPC) from a large dataset to approximate full dataset training with minimal performance loss. While effective in very small IPC ranges, many distillation methods become less effective, even underperforming random sample selection, as IPC increases. Our examination of state-of-the-art trajectory-matching based distillation methods across various IPC scales reveals that these methods struggle to incorporate the complex, rare features of harder samples into the synthetic dataset even with the increased IPC, resulting in a persistent coverage gap between easy and hard test samples. Motivated by such observations, we introduce SelMatch, a novel distillation method that effectively scales with IPC. SelMatch uses selection-based initialization and partial updates through trajectory matching to manage the synthetic dataset's desired difficulty level tailored to IPC scales. When tested on CIFAR-10/100 and TinyImageNet, SelMatch consistently outperforms leading selection-only and distillation-only methods across subset ratios from 5% to 30%.

==> section/conclusion.tex <==

\section{Conclusion}

To address the limitations of current distillation methods, which struggle to scale effectively with increasing IPC,  we introduced SelMatch, a novel distillation method that combines selection-based initialization with partial updates through trajectory matching. Our approach ensures that the distillation process begins with images at an optimized difficulty level, tailored to the specific IPC regime. Moreover, through partial updates, it maintains the unique features of some real samples in the unchanged portion of the synthetic set. Meanwhile, the representative features of a whole dataset are translated through distillation to the rest of the images.
SelMatch sets a new benchmark in performance, outperforming traditional dataset distillation and sample selection methods across various subset ratios on the CIFAR-10/100 and Tiny ImageNet datasets.


%In this paper, we find that the existing dataset distillation methods overly focuses on the simpler, more representative features of the dataset and does not incorporate complex patterns of hard samples in the dataset, resulting in less effective performance scaling even with the increased IPC. To address this limitation, we propose a new distillation method, SelMatch, with selection-based initialization and partial updates through trajectory matching. Selection-based initialization ensures that subsequent distillation process starts with images of an optimized difficulty level for the specific IPC regime, and partial updates while partial updates ensure that unique features of some real samples are preserved within the unaltered portion of the synthetic set. Our method establishes a new state-of-the-art, surpassing both dataset distillation and sample selection methods on the CIFAR-10/100 and Tiny ImageNet benchmarks across 5 to 30\% selection ratios. 



==> section/main_figure.tex <==
\begin{figure*}[t]
  \begin{center}
      \includegraphics[width=\linewidth]{images/illust_all.pdf}
  \end{center}
  \caption{Illustration of our select-and-match method, SelMatch. Our method comprises two key components: 1) Selection-based initialization: SelMatch employs our sliding-window algorithm to select a subset of a suitable difficulty level, initializing the synthetic dataset $\mathcal{D}_\textrm{syn}$ with this chosen subset; 2) Partial update: SelMatch freezes (1-$\alpha$) fraction of samples ($\mathcal{D}_\textrm{select}$) and update only $\alpha$ fraction of samples ($\mathcal{D}_\textrm{distill}$) while minimizing the matching loss $\mathcal{L}( \mathcal{D}_\textrm{select}\cup \mathcal{D}_\textrm{distill}, \mathcal{D}_\textrm{real})$ to preserve unique features of selected real samples.}
  \label{fig:main}
\end{figure*}

% width=.95\linewidth
% height=5 cm

==> section/table_backup.tex <==
\begin{table*}[t]
\centering\scriptsize
\begin{adjustbox}{max width=\linewidth}
\begin{threeparttable}
\caption{Performance of SelMatch compared to other baselines on CIFAR-10, CIFAR-100 and Tiny ImageNet. We highlight the best result across all methods in bold and underline the best result among selection-only baselines. \DAG denotes the use of distilled dataset provided by the original paper without reproduction. For all subset ratios, we set the number of training steps to be 25\% of that with full dataset for 200 epochs.  For the full dataset, we also report the test accuracy measured by training for the full 200 epochs in bracket.}
\label{tab:main_result}
\vskip 0.15in
\centering
\begin{tabular}{c|cccc|cccc|cccc}
\toprule
Dataset & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{CIFAR-100} & \multicolumn{4}{c}{Tiny ImageNet} \\
IPC & 250 & 500 & 1000 & 1500 & 25 & 50 & 100 & 150 & 50 & 100 & 150 & 200 \\
Ratio & $5\%$ & $10\%$ & $20\%$ & $30\%$ & $5\%$ & $10\%$ & $20\%$ & $30\%$ & $10\%$ & $20\%$ & $30\%$ & $40\%$ \\
\midrule
Random & 73.4$\pm$1.5 & 79.3$\pm$0.3 & 85.6$\pm$0.4 & 88.3$\pm$0.2 & 35.8$\pm$0.6 & 40.7$\pm$1.0 & 53.2$\pm$0.9 & 60.3$\pm$1.3 & 30.1$\pm$0.6 & 40.1$\pm$0.4 & 45.7$\pm$0.7 & 48.5$\pm$0.4 \\
Forgetting & 30.9$\pm$0.4 & 41.2$\pm$0.9 & 68.5$\pm$1.5 & 83.1$\pm$0.7 & 8.2$\pm$0.3 & 11.9$\pm$0.6 & 25.7$\pm$0.5 & 41.1$\pm$1.0 & 5.7$\pm$0.1 & 12.4$\pm$0.2 & 22.2$\pm$0.4 & 31.7$\pm$0.5 \\
Glister & 46.6$\pm$1.3 & 56.6$\pm$0.5 & 79.0$\pm$0.7 & 85.0$\pm$0.9 & 21.7$\pm$0.8 & 26.7$\pm$1.3 & 39.9$\pm$1.4 & 52.1$\pm$1.3 & 22.6$\pm$0.5 & 34.0$\pm$0.3 & $\pm$ & $\pm$ \\
Oracle window & \underline{79.3$\pm$0.7} & \underline{85.2$\pm$0.1} & \underline{89.9$\pm$0.5} & \underline{90.6$\pm$0.3} & \underline{43.2$\pm$1.8} & \underline{50.0$\pm$0.8} & \underline{59.2$\pm$0.8} & \underline{64.7$\pm$0.5} & \underline{42.5$\pm$0.3} & \underline{49.2$\pm$0.3} & \underline{52.2$\pm$0.3} & \underline{53.9$\pm$0.2} \\
\midrule
DSA\tnote{1} & 74.7$\pm$1.5 & 78.7$\pm$0.7 & 84.8$\pm$0.5 & - & - & 42.6$\pm$0.5\DAG & - & - & 27.8$\pm$1.4\DAG & - & - & - \\
DM\tnote{1} & 75.3$\pm$1.4 & 79.1$\pm$0.6 & 85.6$\pm$0.5 & - & - & 42.6$\pm$0.5\DAG & - & - & 31.0$\pm$0.6\DAG & - & - & - \\
MTT\tnote{2} & 80.7$\pm$0.4 & 82.2$\pm$0.4 & 86.1$\pm$0.3 & 88.6$\pm$0.2 & 49.9$\pm$0.7 & 51.3$\pm$0.4 & 58.7$\pm$0.6 & 63.1$\pm$0.3 & 40.3$\pm$0.3 & 44.2$\pm$0.5 & x$\pm$x & 50.5$\pm$0.1 \\
FTD\tnote{3,4} & 78.8$\pm$0.2 & 80.0$\pm$0.7 & 85.6$\pm$0.2 & 87.8$\pm$0.4 & 47.4$\pm$0.2 & 49.0$\pm$0.2 & 56.2$\pm$0.3 & 61.0$\pm$0.5 & 30.2$\pm$0.3 & 36.9$\pm$0.6 & $\pm$ & $\pm$ \\
DATM\tnote{3} & - & 84.8$\pm$0.3\DAG & 87.6$\pm$0.3\DAG & - & - & 51.0$\pm$0.5\DAG & 61.5$\pm$0.3\DAG & - & \textbf{42.2}$\pm$\textbf{0.2}\DAG & - & - & - \\
\midrule
SelMatch(ours) & \textbf{82.8}$\pm$\textbf{0.2} & \textbf{85.9}$\pm$\textbf{0.2} & \textbf{90.4}$\pm$\textbf{0.2} & \textbf{91.3}$\pm$\textbf{0.2} & \textbf{50.9}$\pm$\textbf{0.3} & \textbf{54.5}$\pm$\textbf{0.6} & \textbf{62.4}$\pm$\textbf{0.6} & \textbf{67.4}$\pm$\textbf{0.2} & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
\midrule
Full Dataset & \multicolumn{4}{c|}{93.2$\pm$0.3 (95.0$\pm$0.2)} & \multicolumn{4}{c|}{73.9$\pm$0.2 (76.5$\pm$0.7)} & \multicolumn{4}{c}{58.5$\pm$0.3 (61.1$\pm$0.2)} \\
\bottomrule
\end{tabular}
\vskip -0.1in
\begin{tablenotes}
    \item [1] We reproduce DSA and DM only on the scalable regime, CIFAR-10 with IPC ranging from 250 to 1000, following dc-benchmark \cite{dcbench}.
    \item [2] We reproduce MTT with ConvNet-BN and with larger max start epoch $T^+$ than used in the original paper. 
    \item [3] ZCA whitening is used in FTD and DATM.
    \item [4] EMA (exponential moving average) is used in FTD.
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table*}
